Non-Linear Analog Processing in MIMO Systems with Coarse Quantization

Analog to digital converters (ADCs) are a major contributor to the power consumption of multiple-input multiple-output (MIMO) receivers in large bandwidth millimeter-wave systems. Prior works have considered two mitigating solutions to reduce the ADC power consumption: i) decreasing the number of ADCs via analog and hybrid beamforming, and ii) decreasing the ADC resolution, i.e., utilizing one-bit and few-bit ADCs. These mitigating solutions lead to performance loss in terms of achievable rates due to increased quantization error. In this work, the use of nonlinear analog operators such as envelope detectors and polynomial operators, prior to sampling and quantization is considered, as a way to reduce the aforementioned rate-loss. The receiver architecture consists of linear combiners, nonlinear analog operators, and few-bit ADCs. The fundamental performance limits of the resulting communication system, in terms of achievable rates, are investigated under various assumptions on the set of implementable analog operators. Extensive numerical evaluations are provided to evaluate the set of achievable rates and the power consumption of the proposed receiver architectures. Circuit simulations and measurement results, based on both 22 nm FDSOI CMOS technology and 65 nm Bulk CMOS transistor technologies, are provided to justify the power efficiency of the proposed receiver architectures.

==> appendicies.tex <==

\begin{appendices}
    \section{Proof of Proposition \ref{Prop:1}}
    \label{App:Prop1}
Let $n_q= \lfloor\frac{P_{ADC}}{2\alpha}\rfloor$.
For a given quantizer with associated code $\mathcal{C}$, the high SNR achievable rate is $\log{|\mathsf{P}|}= \log{|\mathcal{C}|}$. So, finding the capacity is equivalent to finding the maximum $|\mathcal{C}|$ over all choices of $Q(\cdot)$.
First, let us prove the converse result. Note that $|\mathcal{C}|\leq 2n_q$ since $\mathbf{c}_0=\mathbf{c}_{2n_q}$. The reason is that for the absolute value function $f_{a_j,j}(\cdot),j\in [n_q]$, we have $\lim_{y\to \infty}f_{a_j,j}(y)=\lim_{y\to -\infty}f_{a_j,j}(y)= \infty $. So, 
\begin{align}
\label{eq:lim}
    c_{0,j}=\lim_{y\to -\infty} \mathbbm{1}(f_{a_j,j}-t_j>0)=\lim_{y\to \infty} \mathbbm{1}(f_{a_j,j}-t_j>0)=c_{2n_q,j}.
\end{align}
As a result, $\log{|\mathcal{C}|}\leq 1+\log{n_q}$. Next, we prove achievability.
Let $t_j=\frac{n_q+1}{2}, j\in [n_q]$ and $f_{a_j,j}(y)\triangleq |y-j-\frac{n_q+1}{2}|, j\in [n_q]$, so that the roots of $f_{a_j,j}(\cdot)-t_j$ are $j$ and $j-n_q-1$. Then, $(r_1,r_2,\cdots,r_{2n_q})\!=\!(-n_q,-n_q\!+\!1,\cdots,-1,1,2,\cdots, n_q)$ and \begin{align*}
    c(i,j)=
    \begin{cases}
    1-\mathbbm{1}(j\leq i)\qquad& \text{if }\quad  i\leq n_q,\\
    \mathbbm{1}(n_q-j+1\leq i-n_q) & \text{otherwise}.
    \end{cases}
\end{align*}
For instance, for $n_q=3$, we have $\mathcal{C}=(111,011,001,$ $000,001,011,111)$. Hence, the only repeated codewords are $\mathbf{c}_0$ and $\mathbf{c}_{2n_q}$. As a result, $|\mathcal{C}|=2n_q$, and $\log{|\mathcal{C}|}=1+\log{n_q}$ is achievable. 
\qed

\section{Proof of Theorem \ref{th:1}}
\label{App:th:1}
We provide an outline of the proof. Note that the input alphabet has at most $2n_q+1$ mass points since
based on the proof of Proposition \ref{Prop:1}, the channel output can take at most $2n_q$ values. Let the quantized channel output be denoted by $\widehat{Y}$.
Since the conditional measure $P_{\widehat{Y}|X}(\cdot|x), x\in\mathbb{R}$ is continuous in $x$, and $\lim_{x\to \infty} P_{\widehat{Y}|X}(\mathcal{A}|x) = \mathbbm{1}(\hat{y}\in \mathcal{A}), \mathcal{A}\in \mathbb{B}$ for some fixed $\hat{y}$, the conditions in the proof of \cite[Prop. 1]{singh2009limits} hold, and the optimal input distribution has bounded support. From the extension of Witsenhausen's result \cite{witsenhausen1980some} given in \cite[Prop. 2]{singh2009limits}, the optimal input distribution is discrete and takes at most ${2n_q+1}$ values. This completes the proof of converse. To prove achievability, it suffices to show that one can choose the set of functions $f_{a_j,j}(\cdot), j\in [n_q]$ and quantization thresholds $t_j, j\in [n_q]$ such that the resulting quantizer operates as described in the theorem statement, i.e., it generates $\widehat{Y}=Q(hX+N)$ where $Q(y)=k$ if $y\in [t_{k},t_{k+1}], k\in \{1,\cdots,2n_q]$ and $Q(y)=0$ if $y>t_{2n_q}$ or $y<t_{1}$. To this end, let $\mathbf{t}^*$ be the optimal quantizer thresholds in \eqref{eq:th:1}. Let $r_1,r_2,\cdots,r_{2n_q}$ be the elements of $\mathbf{t}^*$ written in non-decreasing order. Define a quantizer with associated analog functions $f_{a,j}(y)\triangleq  |y-\frac{r_j+r_{n_q+j}}{2}|$ and $t_j=\frac{r_{n_q+j}-r_j}{2}$. Note that $t_j>0$ since $r_j, j\in [n_q]$ are non-decreasing. Then, similar to the proof of Proposition \ref{Prop:1}, the quantization rule gives distinct outputs for $y\in [r_{k},r_{k+1}], k\in \{1,\cdots,2n_q]$ and $y\in [r_{2n_q},\infty) \cup [-\infty,r_{1}]
$ as desired.
\qed

\section{Proof of Proposition \ref{Prop:3}}
\label{App:Prop:3}
For $j\in [n_q]$ and non-decreasing vector $(r_{i_1},r_{i_2},\cdots, r_{i_{2^\delta}})$ where $i_\lambda\in \mathcal{I}_j, j\in [n_q], \lambda\in [2^{\delta}]$, define 
\begin{align*}
&a_{1,j}\triangleq  \frac{r_{i_1}+r_{i_{2^{\delta}}}}{2}, \qquad a_{s,j}\triangleq  \frac{r_{i_{2^{\delta}}}+r_{i_{\eta_s}}}{2}-\sum_{s'=1}^{s-1} a_{s',j}, 1<s\leq \delta,\\
 &t_{j}\triangleq r_{i_{2^{\delta}}}-\sum_{s'=1}^{\delta-1} a_{s',j}, 1<s\leq \delta
\end{align*}
where $\eta_s\triangleq 2^{\delta}- \sum_{s'=1}^{s-1}2^{\delta-s'}+1, s>1$. 
Consider a  quantizer $Q(\cdot)$ with ADC thresholds  $t(1:n_q)$ and associated analog functions $f_{j}(y)\triangleq A_{\delta}(x,a^{\delta}), j\in [n_q]$. Then, $r_1,r_2,\cdots, r_{\gamma}$ are the non-decreasing sequence of roots of $f_{j}(\cdot), j\in [n_q]$, and the associated code of the quantizer $Q(\cdot)$ is $\mathcal{C}$ as desired.
\qed

\section{Proof of Proposition \ref{Prop:6}}
\label{App:Prop:6}
\label{App:Prop:4}
We provide an outline of the proof.  Let us consider the following cases:
\\\textbf{Case 1:} $\sum_{j=1}^{n_q }\kappa_j\geq 2^{n_q}$
\\In this case, one can use a balanced Gray code \cite{bhat1996balanced} to construct $\mathcal{C}$. A balanced Gray code is a (binary) code where consecutive codewords have Hamming distance equal to one, and each of the bit positions changes value either $2\floor{\frac{2^{n_q}}{2n_q}}$ times or $2\ceil{\frac{2^{n_q}}{2n_q}}$ times. If $\min_{j\in [n_q]} \kappa_j\geq 2\ceil{\frac{2^{n_q}}{2n_q}}$ the proof is complete as one can concatenate the balanced gray code with a series of additional repeated codewords to satisfy the transition counts, and since the balanced gray code is a subcode of the resulting code, we have $|\mathcal{C}|=2^{n_q}$. Otherwise,  there exists $j\in [n_q]$ such that $\kappa_j< 2\ceil{\frac{2^{n_q}}{2n_q}}$.
In this case, without loss of generality, let us assume that $\kappa_1\leq \kappa_2,\cdots \leq \kappa_{n_q}$. Note that since $|\kappa_j-\kappa_j'|\leq 2, j,j'\in [n_q]$ and $\kappa_j, j\in [n_q]$ are even, there is at most one $j^*\in [n_q]$ such that $\kappa_{j^*}\leq \kappa_{j^*+1}$. Let $\kappa'_1,\kappa'_2,\cdots,\kappa'_{n_q}$ be the transition count sequence of a balanced gray code $\mathcal{C}'$ written in non-decreasing order. 
Note that $2\ceil{\frac{2^{n_q}}{2n_q}}-2\floor{\frac{2^{n_q}}{2n_q}}=2$. Hence, similar to the above argument, there can only be one $j'\in [n_q]$ for  which   $\kappa_{j'}\leq \kappa_{j'+1}$. 
Since $\sum_{j=1}^{n_q} \kappa_j\geq  2^{n_q}= \sum_{j=1}^{n_q} \kappa'_j$, we must have $j^*\leq j'$. So, the balanced gray code can be used as a subcode similar to the previous case by correctly ordering the bit positions to match the order of $\kappa_j, j\in [n_q]$. This completes the proof. 
\\\textbf{Case 2:} $\sum_{j=1}^{n_q}\kappa_j< 2^{n_q}$
\\The proof is based on techniques used in the construciton of balanced Gray codes \cite{bhat1996balanced}.
We prove the result by induction on $n_q$.
The proof for $n_q=1,2$ is straightforward and follows by construction of length-one and length-two sequences. For $n_q>2$, Assume that the result holds for all $n'_q\leq n_q$. Without loss of generality, assume that $\kappa_1\leq \kappa_2,\leq \cdots \leq \kappa_{n_q}$. The proof considers four sub-cases as follows.
\\\textbf{Case 2.i:} $\sum_{j=3}^{n_q}\kappa_j\in [0,2^{n_q-2}]$
\\In this case, by the induction assumption, there exists $\mathcal{C}'$,  a code with codewords of length $n_q-2$, whose transition sequence is $\kappa_3,\kappa_4,\cdots,\kappa_{n_q}$, and $|\mathcal{C}'|= \sum_{j=3}^{n_q}\kappa_j$. We construct $\mathcal{C}$ from $\mathcal{C}'$ as follows. Let $\mathbf{c}_{0}=(0,0,\mathbf{c}'_0)$, $\mathbf{c}_{1}=(0,1,\mathbf{c}'_0)$, $\mathbf{c}_{2}=(1,1,\mathbf{c}'_0)$,
$\mathbf{c}_{3}=(1,0,\mathbf{c}'_0)$,
$\mathbf{c}_{4}=(1,0,\mathbf{c}'_1)$,
$\mathbf{c}_{5}=(0,0,\mathbf{c}'_1)$, $\mathbf{c}_{6}=(0,1,\mathbf{c}'_1)$,
$\mathbf{c}_{7}=(1,1,\mathbf{c}'_1)$,$\cdots$. This resembles the procedure for constructing balanced gray codes \cite{bhat1996balanced}. We continue concatenating the first two bits of each codeword in $\mathcal{C}$ to the codewords in $\mathcal{C}'$ using the procedure described above until $\kappa_1$ transitions for position 1 and $\kappa_2$ transitions for position 2 have taken place. Note that this is always possible since i) for each two codewords in $\mathcal{C}'$, we `spend' two transitions of each of the first and second positions in $\mathcal{C}$ to produce four new codewords, ii) $\kappa_2-\kappa_1\leq 2$, and iii) $\kappa_2\leq \sum_{j=3}^{n_q}\kappa_j$, where the latter condition ensures that we do not run out of codewords in $\mathcal{C}'$ before the necessary transitions in positions 1 and 2 are completed. After $\kappa_2+1$ codewords, the transitions in positions 1 and 2 are completed, and the last produced codeword is $(0,0,\mathbf{c}'_{\kappa_2+1})$  since $\kappa_1$ and $\kappa_2$ are both even. To complete the code $\mathcal{C}$, we add $(0,0,\mathbf{c}'_{i}), i\in [\kappa_2+2,\sum_{j=3}^{n_q}\kappa_j]$. Then, by construction, we have $|\mathcal{C}|=|\mathcal{C}'|+\kappa_1+\kappa_2=\sum_{j=1}^{n_q}\kappa_j$ and the code satisfied Properties 1), 2), 3), and 5) in Proposition \ref{Prop:2}. 
\\\textbf{Case 2.ii:}$\sum_{j=3}^{n_q}\kappa_j\in [2^{n_q-2}, 2^{n_q-1}]$
\\ Similar to the previous case, let $\mathcal{C}'$ be a balanced gray code with codeword length $n_q-2$ and transition counts $\kappa'_1\leq \kappa'_2\leq \cdots\leq \kappa'_{n_q-2}$. Define $\kappa''_{j}=\kappa_j- \kappa'_{j+2}, j\in \{3,4,\cdots,n_q\}$. Note that $\kappa''_j$ satisfy the conditions on transition counts in the proposition statement, and hence by the induction assumption, there exists a code $\mathcal{C}''$ with transition counts $\kappa''_j, j\in [n_q-2]$. The proof is completed by appropriately concatenating $\mathcal{C}'$ and $\mathcal{C}''$ to construct $\mathcal{C}$. Let $\gamma''$ be the number of codewords in $\mathcal{C}''$ and define $\mathbf{c}_i=(0,0,\mathbf{c}''_i), i\in [\gamma'']$, $\mathbf{c}_{\gamma''+1}=(0,1,\mathbf{c}''_{\gamma''})$,  $\mathbf{c}_{\gamma''+2}=(1,1,\mathbf{c}''_{\gamma''})$, $\mathbf{c}_{\gamma''+3}=(1,0,\mathbf{c}''_{\gamma''})$, $\mathbf{c}_{\gamma''+4}=(1,0,\mathbf{c}'_{1})$,$\cdots$. Similar to the previous case, it is straightforward to show that this procedure yields a code $\mathcal{C}$ with the desired transition sequence. 

The proof for the two subcases where $\sum_{j=3}^{n_q}\kappa_j\in [2^{n_q-1},3 \times 2^{n_q-2}]$ and $\sum_{j=3}^{n_q}\kappa_j\in [3\times 2^{n_q-1}, \times 2^{n_q-1}]$ is similar and is omitted for brevity.

\end{appendices}
